Hierarchical Implicit Models and Likelihood-Free Variational Inference

Implicit probabilistic models are a flexible class of models defined by a simulation process for data. They form the basis for theories which encompass our understanding of the physical world. Despite this fundamental nature, the use of implicit models remains limited due to challenges in specifying complex latent structure in them, and in performing inferences in such models with large data sets. In this paper, we first introduce hierarchical implicit models (HIMs). HIMs combine the idea of implicit densities with hierarchical Bayesian modeling, thereby defining models via simulators of data with rich hidden structure. Next, we develop likelihood-free variational inference (LFVI), a scalable variational inference algorithm for HIMs. Key to LFVI is specifying a variational family that is also implicit. This matches the model's flexibility and allows for accurate approximation of the posterior. We demonstrate diverse applications: a large-scale physical simulator for predator-prey populations in ecology; a Bayesian generative adversarial network for discrete data; and a deep implicit model for text generation.

==> tikz/deep_implicit_model.tex <==
\begin{tikzpicture}

  % Nodes
  \factor[minimum size=0.3cm] {x} {} {} {};
  \factor[above=0.75cm of x, minimum size=0.3cm] {z1} {} {} {};
  \factor[above=0.75cm of z1, minimum size=0.3cm] {z2} {} {} {};
  \node (eps0) [minimum size=0.0cm,right=0.75cm of x] {};
  \node (eps0a) [minimum size=0.0cm,above=0.12cm of eps0.center] {};
  \node (eps0b) [minimum size=0.0cm,below=0.02cm of eps0.center, xshift=-0.2cm] {};
  \node (eps0c) [minimum size=0.0cm,below=0.02cm of eps0.center, xshift=0.2cm] {};
  \draw[] (eps0a.center)--(eps0b.center)--(eps0c.center)--(eps0a.center);
  \node (eps1) [minimum size=0.0cm,right=0.75cm of z1] {};
  \node (eps1a) [minimum size=0.0cm,above=0.12cm of eps1.center] {};
  \node (eps1b) [minimum size=0.0cm,below=0.02cm of eps1.center, xshift=-0.2cm] {};
  \node (eps1c) [minimum size=0.0cm,below=0.02cm of eps1.center, xshift=0.2cm] {};
  \draw[] (eps1a.center)--(eps1b.center)--(eps1c.center)--(eps1a.center);
  \node (eps2) [minimum size=0.0cm,right=0.75cm of z2] {};
  \node (eps2a) [minimum size=0.0cm,above=0.12cm of eps2.center] {};
  \node (eps2b) [minimum size=0.0cm,below=0.02cm of eps2.center, xshift=-0.2cm] {};
  \node (eps2c) [minimum size=0.0cm,below=0.02cm of eps2.center, xshift=0.2cm] {};
  \draw[] (eps2a.center)--(eps2b.center)--(eps2c.center)--(eps2a.center);
  \node[latent, left=0.6cm of z1, minimum size=0.5cm] (beta) {} ;

  \node[right=of x, xshift=-1.15cm, yshift=0.4cm] (xlabel) {$\mbx_n$};
  \node[right=of z1, xshift=-1.15cm, yshift=0.4cm] (z1label) {$\mbz_{n,1}$};
  \node[right=of z2, xshift=-1.15cm, yshift=0.4cm] (z2label) {$\mbz_{n,2}$};
  \node[right=0.04cm of eps0] (eps0label) {$\mbepsilon_{n,0}$};
  \node[right=0.04cm of eps1] (eps1label) {$\mbepsilon_{n,1}$};
  \node[right=0.04cm of eps2] (eps2label) {$\mbepsilon_{n,2}$};
  \node[left=0.04cm of beta] (betalabel) {$\beta$};

  % Edges
  \edge{z1}{x};
  \edge{z2}{z1};
  \edge{eps0}{x};
  \edge{eps1}{z1};
  \edge{eps2}{z2};
  \edge{beta}{x};
  \edge{beta}{z1};
  \edge{beta}{z2};

  % Plates
  \plate[inner sep=0.25cm,xshift=-0.2cm,
    label={[xshift=-15pt,yshift=15pt]south east:$N$}] {plate1} {
    (x)(xlabel)
    (z1)(z2)
    (z1label)(z2label)
    (eps0)(eps1)(eps2)
    (eps0label)(eps1label)(eps2label)
  } {};

\end{tikzpicture}


==> tikz/deep_model.tex <==
\begin{tikzpicture}

  % Nodes
  \node[obs, minimum size=0.5cm] (x)    {} ;
  \node[latent, above=0.75cm of x, minimum size=0.5cm] (z1)    {} ;
  \node[latent, above=0.75cm of z1, minimum size=0.5cm] (z2)    {} ;
  \node[latent, left=0.6cm of z1, minimum size=0.5cm] (beta) {} ;

  \node[right=of x, xshift=-1cm] (xlabel) {$\mbx_n$};
  \node[right=of z1, xshift=-1cm] (z1label) {$\mbz_{n,1}$};
  \node[right=of z2, xshift=-1cm] (z2label) {$\mbz_{n,2}$};
  \node[left=0.04cm of beta] (betalabel) {$\beta$};

  % Edges
  \edge{z1}{x};
  \edge{z2}{z1};
  \edge{beta}{x};
  \edge{beta}{z1};
  \edge{beta}{z2};

  % Plates
  \plate[inner sep=0.25cm,xshift=-0.2cm,yshift=0.1cm,
    label={[xshift=-15pt,yshift=15pt]south east:$N$}] {plate1} {
    (x)(xlabel)
    (z1)(z2)
    (z1label)(z2label)
  } {};

\end{tikzpicture}

